Relative Flatness and Generalization

Flatness of the loss curve is conjectured to be connected to the generalization ability of machine learning models, in particular neural networks. While it has been empirically observed that flatness measures consistently correlate strongly with generalization, it is still an open theoretical problem why and under which circumstances flatness is connected to generalization, in particular in light of reparameterizations that change certain flatness measures but leave generalization unchanged. We investigate the connection between flatness and generalization by relating it to the interpolation from representative data, deriving notions of representativeness, and feature robustness. The notions allow us to rigorously connect flatness and generalization and to identify conditions under which the connection holds. Moreover, they give rise to a novel, but natural relative flatness measure that correlates strongly with generalization, simplifies to ridge regression for ordinary least squares, and solves the reparameterization issue.

==> sec_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Yes, we describe limitations and assumptions in the introduction, as well as at the appropriate positions in the text and discuss broader properties of the results in this paper in the discussion.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{This work contributes to the theoretical understanding of machine learning, in particular deep learning. As such, it has no direct ethical or societal impact. However, this understanding contributes to the trustworthiness of machine learning. Thus, it indirectly impacts the acceptance of automatic decisions made with such models and might facilitate their adoption in critical fields, such as medical applications and autonomous driving.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We have carefully read the ethics review guidelines and confirm that this paper conforms to them.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{We state all assumptions precisely in the introduction and provide further details, interpretations, and all proofs in the appendix.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{The proofs can be found in Appdx~\ref{appdx:proofs}.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Details are in the supplemental material, an implementation is published in a repository at \url{https://anonymous.4open.science/r/RelativeFlatnessAndGeneralization-B175} (anonymized).}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Details are specified in the appendix and the published code contains all training details to reproduce the results.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{In our experiments, we report the individual results of multiple runs and capture variations by reporting the correlation.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{The details are provided in appendix C.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite existing assets we used in our experiments (CIFAR-10 dataset, LeNet5 network, PacBayes-measure implementation). }
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sec_old_featureRobustness_.tex <==

\section{Feature Robustness}\label{sec:featureRobustness}

We consider models $f=(\psi\circ \phi) :\Xcal\rightarrow \Ycal$ that can be decomposed into a feature extraction $\phi:\Xcal \rightarrow \RR^m$ and a model $\psi:\RR^m\rightarrow \Ycal$, which naturally includes standard neural networks due to their layer-wise structure. %as withdepicted in Figure~\ref{fig:functionIllustration}. 
For such models, we define a novel notion of \defemph{feature robustness}, which depends on a small number $\delta>0$, a sample set $S$ and a \defemph{feature selection} defined by a matrix $A\in \RR^{m\times m}$ of \defemph{operator norm} $||A||\leq 1$.  With $\phi_A(x)=\phi(x)(I+A)$ and
\begin{equation}\label{eq:defRobustness}
\begin{split}
\mathcal{F} (f, S, A):= \frac 1{|S|} \sum_{(x,y)\in S} &\Big[ \loss(\psi[ \phi_A(x))],\ y[\phi_A(x)]) -\loss(f(x),y(x))\Big],
%\mathcal{F} (f, S, A):= \frac 1{|S|} \sum_{(x,y)\in S} &\Big[ \loss(\psi[ \phi(x) + A\phi(x)],\ y[\phi(x)+A\phi(x)]) -\loss(f(x),y(x))\Big],
%\mathcal{F} (f, x, A):= \loss(\psi( \phi(x) + A\phi(x)),y(\phi(x) + A\phi(x)))) -\loss(f(x),y),
\end{split}
\end{equation}
%$$\sum_{i=1}^n \beta_i \cdot \mathbb{E}_{A\in\Acal_i}\left [ \mathcal{F}(f,x_i,A) \right ]$$
%$$ \beta_i=  \int_{\{ Ax_i|\ A\in supp\mathcal{A}_i\}} p_\Dcal(x)  dx$$
the definition of feature robustness is given:% as follows:
%
\begin{definition}\label{def:featureRobustness}
Let $\loss:\Ycal\times \Ycal\rightarrow \RR_+$ denote a loss function, $\epsilon$ and $\delta$ two positive (small) real numbers, $S=\{(x_i,y_i)\} \subseteq \Xcal\times \Ycal$ a finite sample set, and $A\in \RR^{m\times m}$ a matrix. A model $f(x)=(\psi\circ \phi)(x)$, which is a composition of functions $\phi:\Xcal \rightarrow \RR^m$ and $\psi:\RR^m\rightarrow \Ycal$, is called $\pmb{\left ( (\delta,S,A),\epsilon\right )}$\defemph{-feature robust}, if $\left |\mathcal{F} (f,S, sA)\right |\leq \epsilon\ \textrm{ for all } 0\leq s\leq \delta.$ \\
More generally, if $\mathcal{A}$ denotes a probability distribution on matrices in $\RR^m$, then we call the model $\pmb{\left ( (\delta,S,\mathcal{A}),\epsilon\right )}$\defemph{-feature robust on average over $\mathcal{A}$}, if 
\[\left | \mathcal{F}(f,S,\Acal) \right | =\left | \Exp{A\sim \mathcal{A}}{ \mathcal{F} (f,S, A)} \right |   \leq \epsilon%\textrm{ for all } 0\leq s\leq \delta.
\]
\end{definition}

The matrix $A$ in feature robustness determines which features shall be perturbed. For each sample, the perturbation is linear in the expression of the feature. Thereby, we only perturb features that are relevant for the output for a given sample and leave feature values unchanged that are not expressed.  For $\phi$ mapping into an intermediate layer of a neural network, traditionally, the activation values of a neuron are considered as feature values, which corresponds to a choice of $A$ as a projection matrix. 
%The feature value $\phi_j(x)$  defined by the $j$-th neuron in the feature space $\phi(x)\in\RR^m$ can be written as $\phi_j(x)=\langle\phi(x), e_j \rangle$, where $e_j$ denotes the $j$-th unit vector and $\langle \cdot,\cdot \rangle$ the scalar product in $\RR^m$. 
However, it was shown by \citet{intriguingProperties} that, for any other direction $v\in \RR^m, ||v||=1$, the values $\langle \phi(x), v \rangle= \textrm{proj}_v \phi(x)$ obtained from the projection $\phi(x)$ onto $v$, can be likewise semantically interpreted as a feature. This justifies the consideration of general \defemph{feature matrices} $A$. 


%Multiplication of $\phi(x)$ with a matrix $A$ corresponds to a weighted selection of $rank(A)$-many features in parallel (e.g., projection matrices on d-dimensional subspaces correspond to the selection of $d$ many features) justifying our terminology considering a matrix $A$ as a feature selection and calling such $A$ a \defemph{feature matrix} in the following. %The same way that, for a sample input $x$, non-activated neurons $\phi_j(x)=0$ are considered as non-expressed features, we call a selection of features defined by matrix $A$ as \defemph{non-expressed} whenever $A\phi(x)=0$.


\paragraph{Distributions on feature matrices induce distributions on the feature space %via multiplication.
}\label{sct:inducingDistributions} Feature robustness is  defined in terms of feature matrices, while the approach exploiting representative data from Section~\ref{sct:representativeness} considers distributions on feature vectors, cf.~\eqref{eq:interpolating}. To connect feature robustness to the notion of $\epsilon$-interpolation, we specify for any distribution $\Acal$ on matrices $A\in \RR^{m\times m}$ an $|S|$-tuple $\Lambda_{\mathcal{A}}=(\lambda_i)$ of probability density functions $\lambda_i$ on the feature space $\RR^m$ with support containing the origin. Multiplication of a feature matrix with a feature vector $\phi(x_i)$ defines a feature direction $A\phi(x_i)$, and for each $z\in \RR^m$ there is some feature matrix $A$ with $\phi(x_i)+z=\phi(x_i)+A\phi(x_i)$ (unless $\phi(x_i)=0)$). Our choice for distributions $\lambda_i$ on $\RR^m$ are therefore distributions that are induced via multiplication of feature vectors $\phi(x_i)\in \RR^m$ with matrices $A\in \RR^{m\times m}$ sampled from a distribution on feature matrices $\Acal$ . Formally, we assume that a Borel measure $\mu_A$ is defined by a probability distribution $\mathcal{A}$ on matrices $\RR^{m\times m}$. We then define Borel measures $\mu_i$ on $\RR^m$ by $\mu_i(C)=\mu_A(\{ A\ |\ A\phi(x_i)\in C\})$ for Borel sets $C\subseteq \RR^m$. Then $\lambda_i$ is the probability distribution defined by the Borel measure $\mu_i$. As a result, we have for each $i$ that
\[ \Exp{A \sim \mathcal{A}}{\loss(\psi(\phi_A(x_i)), y[\phi_A(x_i) ])} =  \Exp{z \sim \lambda_i}{\loss(\psi(\phi(x_i)+  z), y[\phi(x_i)+z])}\]
%\[ \Exp{A \sim \mathcal{A}}{\loss(\psi(\phi(x_i)+  A\phi(x_i)), y[\phi(x_i)+  A\phi(x_i)])} =  \Exp{z \sim \lambda_i}{\loss(\psi(\phi(x_i)+  z), y[\phi(x_i)+z])}\]

\paragraph{Example: Truncated isotropic normal distributions}\hspace{-0.2cm}are induced by a suitable distribution on feature matrices.
%The paper considers an $|S|$-tuple of densities $\Lambda_{\delta,\mathcal{A}}$ induced by  a distribution on feature matrices are truncated scaled normal distributions with support around the training samples. 
We consider probability distributions $\mathcal{K}_{\delta ||\phi(x_i)||}$
%\begin{equation}\label{eq:kernelExample}
%\lambda_i=\mathcal{K}_{\delta||\phi(x_i)||}
%\end{equation} 
on feature vectors $z\in\RR^m$ in the feature space defined by densities $k_{\delta||\phi(x_i)||}(0,z)$ with smooth rotation-invariant kernels, bounded support and bandwidth $h$:
\begin{equation}\label{eq:kernel} k_h(z_i,z)= \frac{1}{h^m}\cdot k \left (\frac{||z_i-z||}{h} \right)  \cdot \mathbbm{1}_{||z_i-z||<h}  \end{equation}
with $\mathbbm{1}_{||z_i-z||<h}=1$ when $||z-z_i||< h$ and $0$ otherwise, and such that $\int_{z\in \RR^m} k_h(z_0,z)\ dz=1\text{ for all $z_0$} .$ 
An example for such a kernel is a truncated isotropic normal distribution with variance $\delta^2 \sigma^2I$, 
$k_h(z_i,z)= \mathcal{N}(z_i, h^2\sigma^2)(z)$.
%\begin{equation}\label{eq:scaledTruncatedGaussians}
%     k_h(z_i,z)= \mathcal{N}(z_i, h^2\sigma^2)(z) =  \frac{C}{h^m} \cdot \exp\left(- \frac{||z-z_i||^2}{h^2\sigma^2}\right )  \cdot \mathbbm{1}_{||z_i-z||<h} 
% \end{equation}
%where $C$ is a normalizing constant, or the truncated multivarite Epanechnikov kernel (see e.g.~\cite{silverman1986density}). 
The following result states that the densities in \eqref{eq:kernel} can indeed be induced by distributions on feature matrices, which will enable us to connect feature robustness with $\epsilon$-representativeness. 

\begin{proposition}\label{prp:lambdaA}
Let $S^\phi=\{\phi(x_i)\ |x_i\in S\}$ be a set of feature vectors in $\RR^m$. With $k_h$ defined as in \eqref{eq:kernel}, let $\lambda_i(z)=k_{\delta||\phi(x_i)||}(0,z)$ define an $|S|$-tuple $\Lambda_{\delta}$ of densities. Then there exists a distribution $\mathcal{A}_\delta$ on matrices in $\RR^{m\times m}$ of norm less than $\delta$
%that induces  each $\lambda_i$ by multiplication with $\phi(x_i)$ so that $\Lambda_{\delta,\mathcal{A}}=\Lambda$.
such that for each $i=1,\ldots,|S|$,
\[ \Exp{A\sim \mathcal{A}_\delta}{  \loss(\psi(\phi_A(x_i)),y[\phi_A(x_i)])}= \mathbb{E}_{\xi \sim \lambda_i}\Big[\loss( \psi(\phi(x_i)+ \xi),y[\phi(x_i)+\xi]) \Big] \]
%\[ \Exp{A\sim \mathcal{A}_\delta}{  \loss(\psi(\phi(x_i)+A\phi(x_i)),y[\phi(x_i)+A\phi(x_i)])}= \mathbb{E}_{\xi \sim \lambda_i}\Big[\loss( \psi(\phi(x_i)+ \xi),y[\phi(x_i)+\xi]) \Big] \]
\end{proposition}

The technical proof is deferred to the appendix, but we describe the distribution $\mathcal{A}_\delta$ on matrices for later use: The desired distribution is defined on the set of matrices of the form $rO$ for a real number $r$ and an orthogonal matrix $O$ (i.e. $OO^T=O^TO=I$) as a product measure combining the (unique) Haar measure on the set of orthogonal matrices $\mathcal{O}(m)$ with a suitable distribution on $\RR$. The Haar measure on $\mathcal{O}(m)$ induces the uniform measure on a sphere of radius $r$ via multiplication with a vector of radius $r$ \citep{Krantz}, and we choose a  measure on $\RR$ to match the radial change of the kernel $k_h$.



\paragraph{Feature robustness and generalization.}
With the above construction, for $\Lambda_{\mathcal{A}_\delta}$ a distribution on the feature space induced by a distribution $\mathcal{A}$ on feature matrices, we have that
\begin{equation}\label{eq:splitError}
\Ecal(f) = \Ecal_{emp}(f,S) + Rep^\phi(f,S,\Lambda_{\mathcal{A}_\delta}) + \mathcal{F}(f,S, \Acal_\delta)
\end{equation}
Here, $\mathcal{A}_\delta$ can be any distribution on feature matrices and can be chosen suitably to control how well the corresponding mixture of local distributions interpolates the true distribution. The third summand is then described by how robust the model is in expectation over feature changes for $A\sim\mathcal{A}_\delta$.   In particular, if $Rep^\phi(f,S,\Lambda_{\mathcal{A}_\delta})\approx 0$, then $\Ecal_{gen}(f,S)\approx \mathcal{F}(f,S, \Acal_\delta)$ and the generalization gap is determined by feature robustness.  



==> sec_old_flatness.tex <==
\section{A connection to flatness of the loss surface}\label{sct:FRandFlatness}
The definition of feature robustness using feature matrices allows us to connect properties in the feature space in neighborhoods around the training points to properties of the weight space and its loss surface using the key equation \eqref{eq:keyEquation}. We repeat here how \eqref{eq:keyEquation} translates to the empirical risk for convenience: For a model $f(x,\w)=\psi(\w,\phi(x))=g(\w\phi(x))$ with parameters $\w\in \RR^{d\times m}$ and $g:\RR^d\rightarrow \Ycal$ an arbitrary twice differentiable function on a matrix product of parameters $\w$ and a feature representation $\phi:\Xcal\rightarrow \RR^m$ and any feature matrix $A\in\RR^{m\times m}$ we have that 
\begin{equation}\label{eq:InputToParameters}
\begin{split}
    \Ecal_{emp}(\w+ \w A,\phi(S)) &=\frac 1{|S|} \sum_{i=1}^{|S|} \loss( \psi (\w+ \w A,\phi(x_i)),y_i) = \frac 1{|S|} \sum_{i=1}^{|S|} \loss(\psi(\w, \phi(x_i)+A\phi(x_i)),y_i) 
\end{split}
\end{equation}
In particular, the performance of a neural network function on perturbed feature vectors can be described by the loss as a function of the weight parameters. This connection between feature robustness and empirical loss surface assumes that the performance for perturbed features is measured with locally constant labels. It can be seen from \eqref{eq:InputToParameters} that, in general, flatness measures of the loss surface that consider the change of the empirical loss as a function of the weights similarly assume locally constant labels. In this section, we introduce a novel, but natural, loss Hessian-based flatness measure that bounds feature robustness. 

%This is the key equation allowing to connect properties in the sample space around training points to the loss as a function of the weight parameters, which can be bounded by flatness measures of the loss surface. For this, let $\loss$ be a loss function and $f(x,\w)=\psi(\phi(x))=g(\w\phi(x))$ be a model with $\w\in \RR^{d\times m}$ and $g:\RR^d\rightarrow \Ycal$ an arbitrary twice differentiable function on a matrix product of parameters $\w$ and the image of $x$ under a feature representation $\phi:\Xcal\rightarrow \RR^m$. Let $\w_i\in\RR^{1\times m}$ denote a row of weight matrix $\w$. 
With $\w_s=(w_{s,t})_t \in \RR^{1\times m}$ denoting the $s$-th row of matrix $\w$, we let $H_{s,s'}(\w,\phi(S))\in\RR^{m\times m}$ denote the Hessian matrix containing all partial second derivatives of the empirical risk $\Ecal_{emp}(\w,\phi(S))$ with respect to weights in rows $\w_s$ and $\w_{s'}$,  i.e. \[H_{s,s'}(\w,\phi(S))=\left [\frac{\partial^2 \mathcal{E}_{emp}(\w,\phi(S))}{\partial w_{s,t} \partial w_{s',t'}} \right ]_{1\leq t,t'\leq m}.\]

\begin{definition}\label{def:flatnessMeasure}
For a model $f(x,\w)=g(\w\phi(x))$, a loss function $\loss$ and a sample set $S$ we define relative flatness measures by
 \begin{equation}\label{eq:defFlatness}
% \kappa^\phi(\w) := \sum_{s=1}^d || \w_s||^2  \cdot \lambda_{max}(H_{s,s}(\w,\phi(S)))\text{ and }
 \kappa^\phi_{Tr}(\w) := \sum_{s,s'=1}^d \langle \w_s,\w_s'\rangle  \cdot Tr(H_{s,s'}(\w,\phi(S))),
\end{equation}
where  $Tr$ denote the  trace and  $\langle \w_s,\w_{s'}\rangle=\w_s\w_{s'}^T$ the scalar product of two row vectors.

%$\lambda_{max}$ and $Tr$ denote the maximal eigenvalue and unnormalized trace respectively and  $\langle \w_s,\w_{s'}\rangle=\w_s\w_{s'}^T$ the scalar product between two row vectors.
\end{definition}

%\begin{definition}\label{def:flatnessMeasure}
%Let $\loss$ be a loss function and $f(x,\w)=\psi(\phi(x))=g(\w\phi(x))$ be a model with $\w\in \RR^{d\times m}$ and $g:\RR^d\rightarrow \Ycal$ an arbitrary twice differentiable function on a matrix product of parameters $\w$ and the image of $x$ under a feature representation $\phi:\Xcal\rightarrow \RR^m$. With $H\mathcal{E}_{emp}(\vvec \w,S)$ denoting the Hessian of the empirical risk as a function of $\w$, we define two relative flatness measures of the loss surface based on the maximal eigenvalue $\lambda_{max}$ and the unnormalized trace $Tr$ as
% \begin{equation}\label{eq:defFlatness}
% \kappa^\phi(\w) := ||\vvec \w||_F^2\cdot \lambda_{max}(H\mathcal{E}_{emp}(\vvec \w,S))\text{ and } \kappa^\phi_{Tr}(\w) := ||\vvec \w||_F^2\cdot Tr(H\mathcal{E}_{emp}(\vvec \w,S)).
%\end{equation}
%\end{definition}


The following theorem shows that relative flatness approximates feature robustness from Definition~\ref{def:featureRobustness} at a local minimum. Section~\ref{sct:flatness} demonstrates additional attractive properties of relative flatness . 

\begin{theorem}\label{thm:averaging}
Consider a model $f(x,\w)=g(\w\phi(x))$ as above, a loss function $\loss$ and a sample set $S$, and let $\delta$ be a positive (small) real number. Let $\w=\omega\in\RR^{d\times m}$ denote parameters at a local minimum of the empirical error on a sample set $S$ and $O_m\subset \RR^{m\times m}$ denote the set of orthogonal matrices. Then, 
%(i) for each feature selection matrix $||A||\leq 1$ the model $f(x,\omega)$ is $\left ( (\delta, S, A), \epsilon \right )$-feature robust for $\epsilon= \frac{\delta^2 d}2 \kappa^\phi(\omega) +\mathcal{O}(\delta^3)$, and  
(%ii)
 $f(x,\omega)$ is $\left ( (\delta, S, O_m), \epsilon \right )$-feature robust on average over $O_m$  for $\epsilon= \frac{\delta^2}{2m} \kappa^\phi_{Tr}(\omega)+\mathcal{O}(\delta^3)$. 
\end{theorem}


\paragraph{Properties of relative flatness}

(i) Relative flatness generalizes Ridge regression for linear models, $f(x,\w)=\w x\in\RR$ ($\Xcal=\RR^d$, $g=id$ and $\phi=id$) and squared loss: To see this, note that for any loss function $\loss$, the second derivatives with respect to the parameters $\w\in \RR^d$ computes to 
$\frac{\partial^2 \loss}{\partial w_i \partial w_j} = \frac{\partial^2 \loss}{\partial (f(x,\w))^2} x_i x_j.$
For $\loss$ the squared loss function, $\sfrac{\partial^2 \loss}{\partial \hat y^2}=2$ and the Hessian is independent of the parameters $\w$. In this case, $\kappa_{Tr}^{id}=c\cdot ||\vvec \w||^2$ with a constant $c=2Tr(xx^t)$, which is (a constant multiple of) the well-known Tikhonov (ridge) regression penalty.

(ii) Invariance under reparameterization: We consider neural network functions \begin{equation}f(x)=\w^L \sigma (\ldots \sigma(\w^2 \sigma(\w^1 x+b^1)+b^2)\ldots )+b^L\end{equation} of a neural network of $L$ layers with nonlinear activation function $\sigma$. 
%We hide a possible non-linearity at the output by integrating it in a loss function $\loss$ chosen for neural network training. 
By letting $\phi^l(x)=\sigma ( \w^{l-1} \sigma (\ldots \sigma(\w^2 \sigma(\w^1 x+b^1)+b^2)\ldots)+b^{l-1})$ denote the output of the composition of the first $l-1$ layers and $g^l(z)=\w^L \sigma (\ldots \sigma(z+b^{l})\ldots )+b^L$ the composition of the activation function of the $l$-th layer together with the rest of layers, we can write for each layer $l$, $f(x,\w^l)=g^l(\w^l \phi^l(x))$. Using \eqref{eq:defFlatness} we obtain for each layer of the neural network a measure of relative flatness with layer weights $\w$. We let $\kappa^l_{Tr}(\w) := \sum_{s,t=1}^d \langle \w^l_s,\w^l_t \rangle \cdot Tr(H_{s,t}(\w,S))$
%\begin{equation}\label{eq:flatnessNetworks}
%    \kappa^l(\w) := \sum_{s=1}^d ||\w^l_{s}||^2 \cdot \lambda_{max}(H_{s,s}(\w^l_s,S)) \text{ and }
%    \kappa^l_{Tr}(\w) := \sum_{s,t=1}^d \langle \w^l_s,\w^l_t \rangle \cdot Tr(H_{s,t}(\w,S))
%\end{equation}
with $Tr$ calculating the  trace of the Hessian of the empirical risk with respect to rows $\w_s^l$ of the parameters of the $l$-th layer denoted by $H_{s,s}$. 

For an everywhere well-defined Hessian of the loss function, we require the network function to be twice differentiable. With the usual adjustments (equations only hold almost everywhere in parameter space), we can also consider neural networks with ReLU activation functions. In this case, \citet{dinhSharp} noted that a linear reparameterization of one layer, $\w^l\rightarrow \lambda \w^l$ for $\lambda>0$, can lead to the same network function by simultaneously multiplying another layer by the inverse of $\lambda$, $\w^k\rightarrow \sfrac 1\lambda \w^k,\ k\neq l$.  Representing the same function, the generalization performance remains unchanged, but this linear reparameterization changes the common measures of the Hessian of the loss, which constitutes an issue in relating flatness to generalization. Our measure fixes this issue since the change of the loss Hessian is counteracted by multyplying with the scalar products of weight matrices and is therefore invariant under layer-wise reparameterizations.  There exist more general neuron-wise reparameterizations that leave the network function unchanged, where we multiply all incoming weights into a neuron by a positive number $\lambda$ and multiply all outgoing weights by $\frac 1\lambda$.  Our relative flatness measure is also independent of such reparameterizations after a simple preprocessing step. 

%of the two subnetworks $\phi^l(\w^1,b^1,\ldots,\w^{l-1},b^{l-1})$ and $\psi^l(\w^l,b^l,\ldots,\w^L,b^L)$ respectively. A neuron-wise reparameterization of the layer $l$, however, changes the representation $\phi^l$, hence it changes both $\epsilon$-interpolation and feature robustness, which results in a change of flatness. One possibility to accommodate this is to consider a different distribution $\mathcal{A}$ on feature matrices such that $\epsilon$-interpolation and feature robustness remain unchanged, but then the tracial measure has to be adjusted accordingly. Instead, we first apply a neuron-wise reparameterization on $\w^{l-1}$ and $\w^l$ to enforce each vector component of  $\phi^l(x_i)$  to have unit variance over samples $x_i$ before measuring relative flatness, which ensures invariance under neuron-wise reparameterizations.


%\begin{theorem}\label{thm:invarianceAll}
%Let $f=f(\w^1,b^1,\w^2,b^2,\ldots, \w^L,b^L)$ denote a neural network function parameterized by parameters $\w^l=w^l_{s,t}$ and bias $b^l_s$ of the $l$-th layer. Suppose there are positive numbers $\lambda_{s,t}^l$ such that the parameters $\w_\lambda^l,b^l_\lambda$, obtained from multiplying $\text{w}_{s,t}^l$ at matrix position $(s,t)$ in layer $l$ by $\lambda_{s,t}^l$ and $b^L_s$ by $\lambda_{(s,0)}^l$, satisfy that $f(\w^1,b^1,\w^2,b^2,\ldots, \w^L,b^L)= f(\w_\lambda^1,b_\lambda^1,\w_\lambda^2,b_\lambda^2,\ldots, \w_\lambda^{L}, b_\lambda^L)$. If for some $l$ it holds that $\lambda^l_{(s,t)}=\lambda^l_{(s,t')}$ for each $s,t$ and $t'$, then $\kappa^l(\w)=\kappa^l(\w_\lambda)$ and $\kappa^l_{Tr}(\w) =\kappa^l_{Tr}(\w_\lambda)$.
%\end{theorem}

\begin{theorem}
Let $\sigma_i$ denote the variance of the i-th coordinate of $\phi(x;\w^{l-1},b^{l-1},\ldots,\w^1,b^1)$ over 
samples $x\in S$ and $V=diag\left ( {\sigma_1},\ldots, {\sigma_{n_{l-1}}}\right )$. If the relative flatness measure $\kappa^l_{Tr}$ is applied to \[f=\psi(\w^lV,b^l,\w^{l+1},b^{l+1}\ldots, \w^L,b^L) \circ  \phi(V^{-1}\w^{l-1},V^{-1}b^{l-1},\ldots,\w^1,b^1),\]
then $\kappa^l_{Tr}$ is invariant under all neuron-wise (and layer-wise) reparameterizations 
\end{theorem}




==> sec_old_flatnessAndGeneralization.tex <==


\section{Flatness and generalization}
Combining the results from Sections~\ref{sct:representativeness}--\ref{sct:FRandFlatness}, we obtain a generalization bound that holds uniformly over all distributions that can be represented by smooth probability densities on a feature space with with \textcolor{blue}{approximately} locally constant labels. 

\textcolor{red}{TO DISCUSS WHICH VERSION OF THE THEOREM TO ADD}
\begin{theorem}\label{thm:FlatnessGenBound}
%Consider a model $f(x,\w)=g(\w\phi(x))$ as above, a loss function $\loss$ and a sample set $S$,  let $m$ denote the dimension of the feature space defined by $\phi$ and let $\delta$ be a positive (small) real number. Let $\omega$ denote a local minimum of the empirical error on a sample set $S$. 
%(i) For any $|S|$-tuple of distribution $\Lambda_{\mathcal{A}_\delta}$ on feature feature vectors induced by a distribution $\mathcal{A}_\delta$ on feature matrices of norm smaller than $\delta$ as in Section~\ref{sct:inducingDistributions}, it holds that  
%\[\Ecal_{gen}(f(\cdot,\omega),S) \leq Int^\phi(f,S,\Lambda_{\mathcal{A}_\delta}) + \frac{\delta^2d}2  \kappa^\phi(\omega)+ \mathcal{O}(\delta^3) \] 
%(ii) Suppose that the distribution $\Dcal$ has a smooth density $p^\phi_\Dcal$ on the feature space $\RR^m$ such that $\int_z  \left | \nabla^2 \left( p^\phi_\Dcal(z)||z||^2\right ) \right | dz $ and $\int_z \frac{p^\phi_\Dcal(z)}{||z||^m}\ dz$ are well-defined and finite. Then for sufficiently large sample size $|S|$, if the distribution has locally constant labels, then it holds with probability $1-\Delta$ over sample sets $S$ that
%\[\Ecal_{gen}(f(\cdot, \omega),S)\lesssim |S|^{-\frac{2}{4+m}} \left ( \frac{\kappa^\phi_{Tr}(\omega)}{2m}  +  C_1(p^\phi_\Dcal,L)+\frac{C_2(p^\phi_\Dcal,L)}{\sqrt{\Delta}} \right ) \] 
%up to higher orders in $|S|^{-1}$ for constants $C_1,C_2$ that depend only on the distribution in feature space $p^\phi_\Dcal$ induced by $\phi$ and the chosen $|S|$-tuple $\Lambda_{\mathcal{A}_\delta}$ and the maximal loss $L$.
Consider a model $f(x,\w)=g(\w\phi(x))$ as above, a loss function $\loss$ and a sample set $S$,  let $m$ denote the dimension of the feature space defined by $\phi$ and let $\delta$ be a positive (small) real number. Let $\omega$ denote a local minimum of the empirical error on a sample set $S$. Suppose that the distribution $\Dcal$ has a smooth density $p^\phi_\Dcal$ on the feature space $\RR^m$ such that $\int_z  \left | \nabla^2 \left( p^\phi_\Dcal(z)||z||^2\right ) \right | dz $ and $\int_z \frac{p^\phi_\Dcal(z)}{||z||^m}\ dz$ are well-defined and finite. Then for sufficiently large sample size $|S|$, if the distribution has locally constant labels, then it holds with probability $1-\Delta$ over sample sets $S$ that
\[\Ecal_{gen}(f(\cdot, \omega),S)\lesssim |S|^{-\frac{2}{4+m}} \left ( \frac{\kappa^\phi_{Tr}(\omega)}{2m}  +  C_1(p^\phi_\Dcal,L)+\frac{C_2(p^\phi_\Dcal,L)}{\sqrt{\Delta}} \right ) \] 
up to higher orders in $|S|^{-1}$ for constants $C_1,C_2$ that depend only on the distribution in feature space $p^\phi_\Dcal$ induced by $\phi$ and the chosen $|S|$-tuple $\Lambda_{\mathcal{A}_\delta}$ and the maximal loss $L$.

\end{theorem}

Part (i) of the theorem states that when the data can be well-approximated in feature space by distributions $\Lambda_{\mathcal{A}_\delta}$ constructed as in Section~\ref{sct:inducingDistributions} and locally constant labels, i.e. $Int^\phi(f,S,\Lambda_{\mathcal{A}_\delta})\approx 0$ for some distribution on feature matrices $\Acal_\delta$ ofr norm smaller than $\delta$, then relative flatness governs the generalization gap. This could explain the often observed correlation between flatness and generalization when real-world data distributions enable $\epsilon$-interpolation for small $\epsilon$, since in this case flatness is the main contributor to the generalization gap. In particular for image classification, the possibility to approximate with locally constant labels may be a reasonable assumption.

In part (ii) we use that common distributions used in kernel density estimation fall into the class of distributions $\Lambda_{\mathcal{A}_\delta}$ as shown in Proposition~\ref{prp:lambdaA}. The term quantifying $\epsilon$-interpolation in (i) aims to approximately cover the data distribution by distributions with localized support of volume governed by $\delta$, hence an increasing sample size $N$ allows for smaller $\delta$ to bound representativeness and hence the generalization bound tends to zero. %
Part (ii) quantifies this convergence for the tracial version of relative flatness for a specific distribution $\mathcal{A}$ on feature matrices. 

We discuss the limitations of part (ii) in the theorem. Our bound suffers from the curse of dimensionality\footnote{Our convergence rate is consistent with the no free lunch theorem and the convergence rate derived by \citet{belkinPerfectFit} in the interpolation regime for an interpolation technique using nearest neighbors with $\alpha=2$}, but for the chosen feature space instead of the (usually much larger) input space. We argue in Section~\ref{} that it follows from the no-free-lunch theorem that a dependence on the dimension is the expected behavior to finding non-vacuous generalization bounds in the interpolation regime uniformly over all smooth distributions $\Dcal$. Further, as a uniform bound, the constants may be large, limiting the influence of the tracial measure in the bound, for wild distributions that can not be well-approximated to exhibit small $\epsilon$-interpolation. Better bounds for the interpolation regime could be achieved by restricting the set of allowed true data distribution. Both, the dimension-dependent convergence rate and the general constants in (ii) are consequences of estimating $\epsilon$-interpolation uniformly for arbitrarily bad smooth data distributions. The quantification of $\epsilon$-interpolation in practical applications is an interesting direction for future work. 



==> sec_old_introduction.tex <==
\section{Introduction}
It has been observed that traditional computational learning theory does not explain the performance of modern machine learning algorithms~\citep{understandingRethinking,bartlett2020benign, nagarajan2019uniform, belkin2018understand}.
This is captured in the ``double descent'' picture  \citep[see][Fig.~1]{belkin2019reconciling} where we distinguish between the \textit{approximation regime} (under-parameterization) where the model capacity is so low that the training data is only approximated and the \textit{interpolation regime} (over-parameterization) where the model capacity is high enough that the training data is fitted perfectly.

%Here introduction representativeness


Traditional learning theory bounds the generalization gap, i.e., the difference between the general risk and the empirical risk, in the capacity of the model class.
Thus, by design, these approaches only yield meaningful bounds in the approximation regime. 

In this paper, we provide an approach to bound the generalization gap that remains meaningful in the interpolation regime, which implies a changed trade-off.
A celebrated feature of traditional bounds 
%for the approximation regime 
is that they do not require any assumption on the underlying data distribution.
Unfortunately, this feature has to be sacrificed in the interpolation regime because the model capacity is too large to bound the generalization gap and the empirical risk provides in itself no implication to the population risk for arbitrary distributions (no-free-lunch theorem~\citep[cf.][Thm~5.1]{learningTheoryBook}).
On the positive side, embracing distribution-dependence leads us to \textit{algorithm-agnostic} bounds for a particular model at hand, independent of the learning algorithm's explicit or implicit inductive bias and its effect on the model capacity. This is an important advantage as this bias is difficult to analyze for modern optimization techniques.

\paragraph{(2)} Several approaches consider the loss surface to attempt an explanation of the generalization capabilities of neural networks, where the loss surface is defined as the function mapping parameter settings to the loss that the corresponding model experiences \cite{}. It has been empirically observed that the generalization performance of a model correlates with the flatness of the loss surface, where local minima generalize better if they fall into flat minima as measured by the size of eigenvalues of the Hessian matrix containing partial second derivatives of the empirical loss function with respect to weight parameters. 

\paragraph{(3)} However, the precise relation is still mysterious and recent research \cite{Dinh, Flatness_False_Friend} rather concentrates on cases where the relation seemingly breaks down, at least  for purely Hessian-based measures of flatness. This raises the question how a correlation could have been observed in the first place. 

\paragraph{(4)} In particular, \citet{Dinh} show that there exist reparameterizations of ReLU-networks that alter Hessian-based flatness arbitrarily but leaves the network function unchanged. Subsequently, reparameterization-invariant measures have been proposed \cite{Rang??, tsuzuku, fisher-rao}, but the theoretical connection to generalization remains still unsolved. 

\paragraph{(5)} The starting point to our investigations is the desire to explain the relation between Hessian-based flatness and generalization in a rigorous and analytical way. 

\paragraph{(6)} We will throughout consider Hessian-based flatness in terms of the spectrum of the loss Hessian and derive our own measure based on it. By definition, flatness is then a local property of the loss surface describing how the model reacts to a local change of parameters for the fixed set of training samples.

\paragraph{(7)} In contrast, generalization performance depends on how the sample loss deviates from the empirical error for unseen samples for a fixed parameter setting, that is, how much the prediction of the model on some unseen $x\in \Xcal$ deviates from the corresponding label $y\in\Ycal$.

\paragraph{(8)} In any practical scenario, we only know samples $(x_i,y_i)\in S$ and have no access to the information how optimal labels $y_i$ react to changes of the input points $x_i$. However, the choice of a model after training makes assumptions since it can applied to predict a label to any input $x$. 


\paragraph{(9)}
\begin{figure}[t]
	\centering
	\includegraphics[width=\textwidth]{images/overview.png}
	\caption{Overview. We theoretically connect a notion of representative data with a notion of feature robustness and a novel measure of flatness of the loss surface.}
	\label{fig:overview}
\end{figure} Properties of these assumptions are encoded in the flatness properties of the loss surface as the following key equation demonstrates. 
Suppose that we are given a function $f(x,\w)=\psi(\w, \phi(x))=g(\w \phi(x))$, that is composed of a feature function $\phi:\Xcal\rightarrow \RR^m$, of a matrix product with some $\w\in \RR^{d\times m}$, and of a prediction function $g:\RR^d\rightarrow \Ycal$. For neural networks, $\phi$ can describe the map from input to any feature layer of the network, $\w$ the weights of this layer and $\psi$ the rest of the function. 
%Let further $\loss:\Ycal \times \Ycal\rightarrow \RR_+$ denote the loss function for supervised learning and $S=\{(x_i,y_i)\ |\ i=1,\ldots,N\}$ a sample set. In the following, we write $z=\phi(x)$. 
We aim to relate network prediction $\psi(\phi(x)+z,\w)$ at new features $\phi(x)+z$ and fixed parameters $\w$ to the performance at the original features $\phi(x)$ but under changes of the model, which is $\psi(\phi(x),\w+\tilde \w)$. This connection becomes possible by finding a matrix  $A\in\RR^{m\times m}$ such that $z=A\phi(x)$ (which is always possible unless $\phi(x)=0$) as in this case we have that 
\begin{equation}\label{eq:keyEquation}
    \psi(\w, \phi(x)+A\phi(x))=g(\w (\phi(x)+ A\phi(x))) = g((\w+ \w A )\phi(x))=\psi (\w+ \w A,\phi(x))\enspace .
\end{equation} 
If we now consider the loss $\loss$ at a sample $S$ and using \eqref{eq:keyEquation}, we see from
\[\Ecal_{emp}(S, \w+ \w A) =\frac 1n \sum_i \loss( \psi (\w+ \w A,\phi(x_i)),y_i) = \frac 1n \sum_i \loss(\psi(\w, \phi(x_i)+A\phi(x_i)),y_i) \]
that the loss surface is described by the change of the empirical loss under feature perturbations while keeping the labels constant.
\TODO{If we do robustness not on a feature layer but on the input layer, we end up with traditional robustness~\citep{robustnessGeneralization}}

 \paragraph{(10)} Consequently, we are able to connect flatness to generalization by assuming that small changes of features keep labels constant. For this, we propose a novel approach to generalization bounds based on ideas of interpolation and suitable for the interpolation regime.


\paragraph{(11)} We decompose the generalization gap into two terms measuring (i) how representative the sample data is and (ii) how robust the model is to perturbations of its implicitly represented features.

\paragraph{(12)} More concretely, the first term measures how well the true distribution can be approximated by a distribution with support concentrated in a neighborhood of feature vectors of training points and locally constant labels. 

\paragraph{(13)} Since the true data distribution is unknown, this term is hard to estimate, but we show that arguments from kernel density estimation lead to a uniform bound. 

\paragraph{(14)} Our bound suffers from the curse of dimensionality for the feature space dimension and we demonstrate that a variant of the no free lunch theorem implies that this is the best possible result that can be obtained in the interpolarion regime without further restrictions or priors on the true distribution that shift the sample size into the approximation regime. 

\paragraph{(15)} The second term in the decomposition of the generalization gap describes how robust the model is under perturbation of the feature space under the assumption of locally constant labels.  

\paragraph{(16)} A Taylor decomposition at local minima reveals that this term is predominantly determined by Hessian based flatness of the loss surface. We thereby derive a novel flatness measure and show that our measure comes with nice and interpretable properties. 

\paragraph{(17)} Taken together, our results theoretically connect Hessian-based flatness to generalization through novel notions of feature robustness and representativeness. Flatness of the loss surface is described by feature robustness under the assumption of locally constant labels. This suggests that data distributions used in practice can be well-described by locally constant labels in feature space, which offers an explanation why a strong relation between flatness and generalization has been observed empirically.

\paragraph{(18)} Contribution summary

\paragraph{(19)} The paper is organized as follows.

Idea: Replace parts of the introduction to the contributions to keep the discussion shorter


==> sec_old_representativeness.tex <==

\section{Representativeness}\label{sct:representativeness}



We begin by formalizing when a sample set $S$ is representative for a data distribution $\Dcal$.  Since neural networks are deterministic models, they can only model degenerate distributions with deterministic response variable $y$ in $\Ycal$ given $x\in \Xcal$, which entails an unavoidable error on general distributions $\Dcal$. We therefore assume the existence of an optimal label function $y(x)$. Depending on the loss function and learning task, $y(x)$ could be the conditional mean for squared loss in regression or $y(x)$ could be the Bayes classifier for the zero-one loss~\citep[cf.][]{belkinPerfectFit}. The marginal distribution $\Dcal_\Xcal$ on $\Xcal$ and the optimal label $y(x)$ define a degenerate distribution $\Dcal_{Bayes}$ on $\Xcal\times\Ycal$, which we will identify with $\Dcal$. We further assume that the marginal distribution $\Dcal_\Xcal$ is absolute continuous with respect to the Lebesgue measure on $\Xcal$ so that the distribution $\Dcal$ is described by a density function $p_{\Dcal}(x)$. 
%For technical reasons that become apparent later, we assume that $x=0$ is not in the support of $\Dcal$, which we can always achieve by extending the input by one dimension with entry $1$ corresponding to an additive bias term after multiplication with a matrix.


\paragraph{Partitioning the input space.} We choose a partition $\{V_i\ |i=1,\ldots,|S|\}$ of $\Xcal$ such that each element of this partition $V_i$ contains exactly one of the samples $x_i$ from $S$. The distribution can then be described by a set of unnormalized densities $p_i(x)=p_\Dcal(x) \cdot \mathbf{1}_{V_i}(x)$ with support contained in $V_i$ (where $\mathbf{1}_{V_i}(x)=1$ if $x\in V_i$ and $0$ otherwise). With the normalizing factor $\alpha_i=\int_{V_i} p_\Dcal(x)  dx$, %we can write the risk as
%\[\Ecal(f) = \int p_\Dcal(x) \loss(f(x),y(x)) dx = \sum_{i=1}^n \alpha_i \int p_i(x) \loss(f(x),y(x)) dx=  \sum_{i=1}^n \alpha_i \mathbb{E}_{x\sim p_i}[ \loss(f(x,y(x))]. \]
the risk decomposes as $\Ecal(f) = \sum_{i=1}^n \alpha_i\cdot  \mathbb{E}_{x\sim p_i}[ \loss(f(x,y(x))]$, where $\mathbb{E}_{x\sim p_i}$ denotes the expectation over the normalized probability density function $\frac 1\alpha_i \cdot p_i(x)$. 
Since $x_i\in V_i$ for each $i$, we can change variables and consider unnormalized density functions $\lambda_i^*(\xi)=p_i(x_i+\xi)$ with support contained in a neighborhood around $0_\Xcal$. The risk then decomposes as
%\[\Ecal(f)= \int p_\Dcal(x) \loss(f(x),y(x)) dx =  \sum_{i=1}^n \alpha_i \mathbb{E}_{x\sim \lambda_i}[ \loss(f(x_i+x),y(x_i+x))]. \]
\begin{equation}\label{eq:decomposition}
\Ecal(f)=  \sum_{i=1}^n \alpha_i \cdot \mathbb{E}_{\xi\sim \lambda_i^*}[ \loss(f(x_i+\xi),y(x_i+\xi))] %\ \text{ , where }\alpha_i^*=\int_{\Xcal} \lambda_i^*(x)  dx
.\end{equation}
Starting from this identity, we formalize an approximation to the risk. Given a sample set $S$ and an $|S|$-tuple $\Lambda = (\lambda_i)_{1\leq i\leq |S|}$ of ``local'' unnormalized density functions on $\Xcal$ with support  ${supp}(\lambda_i)$ contained in a neighborhood around the origin,  we call the pair $(S,\Lambda)$ \defemph{ $\epsilon$-representative for $\Dcal$} with respect to a model $f$ and loss $\loss$ if $|Rep(f,S,\Lambda) |\leq \epsilon$, where 
\begin{equation}\label{eq:representativeness}
     Rep(f,S,\Lambda)= \Ecal(f)   -\sum_{i=1}^n \beta_i \cdot \mathbb{E}_{\xi\sim \lambda_i}[ \loss(f(x_i+\xi),y(x_i+\xi)),\text{ and } \beta_i=\frac{\int_{\xi}\lambda_i(\xi)\ d\xi }{\sum_i \int_{\xi} \lambda_i(\xi)\ d\xi}
\end{equation}


If the density function $\lambda_i(\xi)=\lambda^*(\xi)$ are all chosen optimal, then $Rep(f,S,\Lambda)=0$. If the support of each $\lambda_i$ is decreased to $0_\Xcal$ so that $\lambda_i=\delta_{0}$, then $Rep(f,S,\Lambda)=\Ecal_{gen}$ is the generalization gap. For density functions with an intermediate support, the generalization gap decomposes into representativeness and a term describing properties of the model around training samples:
\[\Ecal_{gen}(f,S) = Rep(f,S,\Lambda)+  \sum_{i=1}^n \beta_i \cdot \Big (\mathbb{E}_{\xi\sim \lambda_i}[ \loss(f(x_i+\xi),y(x_i+\xi))-\loss(f(x_i),y(x_i))]\Big  )\]
The main idea of our approach to generalization is to take advantage of this equality and to control both representativeness and local properties of the model for a suitable $|S|$-tuple of distributions $\Lambda$
%Formally, given a family $(\lambda_i)_{1\leq i\.leq N}$ of local probability distributions (i.e., with support contained in a $\delta$-neighborhood around the origin) on $\RR^m$, the pair $(S,\Lambda_\delta)$ is called \defemph{ $\epsilon$-representative for $\Dcal$} (in feature space $\RR^m$ with respect to a model $f=(\psi\circ \phi$) and loss $\loss$) if $|Rep(f,S,\Lambda) |\leq \epsilon$, where 
%\begin{equation}\label{eq:representativeness}
%     Rep(f,S,\Lambda)= \Ecal(f)   -\sum_{(x_i,y_i)\in S} \alpha_i \cdot  \displaystyle\mathop{\mathbb{E}}_{\xi \sim \lambda_i}\left[\loss( \psi(\phi(x_i)+ \xi),y(x_i+\xi))\right]
%\end{equation}



%Formally, given a family $(\lambda_i)_{1\leq i\leq N}$ of local probability distributions (i.e., with support contained in a $\delta$-neighborhood around the origin) on $\RR^m$, the pair $(S,\Lambda_\delta)$ is called \defemph{ $\epsilon$-representative for $\Dcal$} (in feature space $\RR^m$ with respect to a model $f=(\psi\circ \phi$) and loss $\loss$) if $|Rep(f,S,\Lambda) |\leq \epsilon$, where 
%\begin{equation}\label{eq:representativeness}
%     Rep(f,S,\Lambda)= \Ecal(f)   -\sum_{(x_i,y_i)\in S} \alpha_i \cdot  \displaystyle\mathop{\mathbb{E}}_{\xi \sim \lambda_i}\left[\loss( \psi(\phi(x_i)+ \xi),y(x_i+\xi))\right]
%\end{equation}

\paragraph{A more practical version.}  The distribution $p_\Dcal$ is unknown and hence, in the decomposition \eqref{eq:decomposition}, we have unknown densities $\lambda_i$, unknown normalization factors $\alpha_i$, and, in the standard setting of machine learning, we do not know how the optimal response variable $y(x_i+\xi)$ changes from $y(x_i)=y_i$. We assume that each neighborhood contributes equally to the loss, i.e., we approximate each $\alpha_i$ with $\frac 1n$. Relying on the information obtained through $S$, we could assume  that $y(x_i)\approx y_i$ int the support of the local distribution $\lambda_i$ for all training samples $(x_i,y_i)\in S$. In fact, this will allow us later to connect generalization to flatness. Alternatively, potential prior assumptions on how labels change in neighborhoods of training points could be applied. We carry on with the more general version and do not make any further restrictions for now. Our revised version of representativeness is given by
\begin{equation}\label{eq:interpolating}
     Rep(f,S,\Lambda)= \Ecal(f)   - \sum_{(x_i,y_i)\in S} \frac 1n\cdot \mathbb{E}_{\xi \sim \lambda_i}\left[\loss( f(x_i+ \xi),y_i(x_i+\xi_i)\right]
\end{equation}



\paragraph{Feature space considerations}An interesting aspect of $\epsilon$-representativeness is that it can be considered in a feature space instead of the input space. For a model $f=(\psi\circ \phi) :\Xcal\rightarrow \Ycal$, we can consider $\phi$ as a feature extractor and $\psi$ as the model, and apply our notion to the feature layer. This leads to the notion of $\epsilon$-representativeness in feature space defined for an $|S|$-tuple $\Lambda^\phi =(\lambda^\phi_i)_{1\leq i\leq N}$ of densities on $\phi(\Xcal)$ by replacing $x_i$ with $\phi(x_i)$ in \eqref{eq:interpolating}, which we denote by  $Rep^\phi(f,S,\Lambda^\phi)$.
%by  
%\begin{equation}\label{eq:representativenessFeature}
%     Int^\phi(f,S,\Lambda^\phi)= \Ecal(f)   -\frac 1n \sum_{(x_i,y_i)\in S} \mathbb{E}_{\xi \sim \lambda_i^\phi}\left[\loss( \psi(\phi(x_i)+ \xi),y_i)\right]
%\end{equation}
We can now decompose the risk  $\Ecal(f)$ of $f=(\psi\circ \phi)$ into
\[ \Ecal_{emp}(f) + Rep^\phi(f,S,\Lambda^\phi) + \left(\frac 1n \sum_{(x_i,y_i)\in S} \mathbb{E}_{\xi \sim \lambda_i^\phi}\left[\loss( \psi(\phi(x_i)+ \xi),y(x_i+\xi_i))- \loss(f(x_i),y_i) \right] \right ) \]
%\begin{wrapfigure}{h}{0.5\textwidth}
%	\centering
%	\input{images/functionIllustration}
%	\caption{Illustration of the decomposition into a feature extractor and a model, i.e., $f=\psi\circ\phi$, for neural networks.}
%	\label{fig:functionIllustration}
%\end{wrapfigure}
The term in the final bracket is determined by how the loss changes under small perturbations in the feature space for the samples in $S$.  As before,  for $\lambda_i=\delta_0$  the term in the bracket vanishes and $Rep^\phi(f,S,\Lambda)=\Ecal_{gen}$.  But the decomposition becomes more interesting for distributions with support of nonzero measure around the origin. %Having trained a neural network to a local minimizer of the empirical error, the term in the bracket is positive for neighborhoods with support of positive measure. 
 If the true distribution can be interpolated efficiently in feature space from the samples in $S$ with suitable $\lambda_i^\phi$ so that  $Rep^\phi(f,S,\lambda)\approx 0$, then the bracket approximately equals the generalization gap and the generalization gap can be estimated from local properties in feature space  around training samples. In the next section, we will define a novel notion of feature robustness of a model that is able to exploit the above connection between $\epsilon$-interpolation and the generalization gap for natural distributions $\Lambda$, 
 %. This notion of feature robustness naturally describes properties of the loss surface as a function of the weight parameters, 
%which finally allows us to connect generalization to a measure of flatness of the loss surface.


==> sec_oldold_featureRobustness.tex <==

\section{Feature Robustness and Flatness of the Loss Curve}\label{sec:featureRobustness}

We consider models $f=(\psi\circ \phi) :\Xcal\rightarrow \Ycal$ that can be decomposed into a feature extraction $\phi:\Xcal \rightarrow \RR^m$ and a model $\psi:\RR^m\rightarrow \Ycal$, which naturally includes standard neural networks due to their layer-wise structure. %as withdepicted in Figure~\ref{fig:functionIllustration}. 
For such models, we define a novel notion of \defemph{feature robustness}, which depends on a small number $\delta>0$, a sample set $S$ and a \defemph{feature selection} defined by a matrix $A\in \RR^{m\times m}$ of \defemph{operator norm} $||A||\leq 1$.  With 
\begin{equation}\label{eq:defRobustness}
\begin{split}
\mathcal{F} (f, S, A):= \frac 1{|S|} \sum_{(x,y)\in S} &\left[ \loss(\psi( \phi(x) + A\phi(x)),y) -\loss(f(x),y)\right],
%\mathcal{F} (f, x, A):= \loss(\psi( \phi(x) + A\phi(x)),y(\phi(x) + A\phi(x)))) -\loss(f(x),y),
\end{split}
\end{equation}
%$$\sum_{i=1}^n \beta_i \cdot \mathbb{E}_{A\in\Acal_i}\left [ \mathcal{F}(f,x_i,A) \right ]$$
%$$ \beta_i=  \int_{\{ Ax_i|\ A\in supp\mathcal{A}_i\}} p_\Dcal(x)  dx$$
the definition of feature robustness is given:% as follows:
%
\begin{definition}\label{def:featureRobustness}
Let $\loss:\Ycal\times \Ycal\rightarrow \RR_+$ denote a loss function, $\epsilon$ and $\delta$ two positive (small) real numbers, $S=\{(x_i,y_i)\} \subseteq \Xcal\times \Ycal$ a finite sample set, and $A\in \RR^{m\times m}$ a matrix. A model $f(x)=(\psi\circ \phi)(x)$, which is a composition of functions $\phi:\Xcal \rightarrow \RR^m$ and $\psi:\RR^m\rightarrow \Ycal$, is called $\pmb{\left ( (\delta,S,A),\epsilon\right )}$\defemph{-feature robust}, if $\left |\mathcal{F} (f,S, sA)\right |\leq \epsilon\ \textrm{ for all } 0\leq s\leq \delta.$ \\
More generally, if $\mathcal{A}$ denotes a probability distribution on matrices in $\RR^m$, then we call the model $\pmb{\left ( (\delta,S,\mathcal{A}),\epsilon\right )}$\defemph{-feature robust on average over $\mathcal{A}$}, if 
\[\left | \mathcal{F}(f,S,\Acal) \right | =\left | \Exp{A\sim \mathcal{A}}{ \mathcal{F} (f,S, A)} \right |   \leq \epsilon%\textrm{ for all } 0\leq s\leq \delta.
\]
\end{definition}

The matrix $A$ in feature robustness determines which features shall be perturbed. For each sample, the perturbation is linear in the expression of the feature. Thereby, we only perturb features that are relevant for the output for a given sample and leave feature values unchanged that are not expressed.  For $\phi$ mapping into an intermediate layer of a neural network, traditionally, the activation values of a neuron are considered as feature values, which corresponds to a choice of $A$ as a projection matrix. 
%The feature value $\phi_j(x)$  defined by the $j$-th neuron in the feature space $\phi(x)\in\RR^m$ can be written as $\phi_j(x)=\langle\phi(x), e_j \rangle$, where $e_j$ denotes the $j$-th unit vector and $\langle \cdot,\cdot \rangle$ the scalar product in $\RR^m$. 
However, it was shown by \citet{intriguingProperties} that, for any other direction $v\in \RR^m, ||v||=1$, the values $\langle \phi(x), v \rangle= \textrm{proj}_v \phi(x)$ obtained from the projection $\phi(x)$ onto $v$, can be likewise semantically interpreted as a feature. This justifies the consideration of general \defemph{feature matrices} $A$. 


%Multiplication of $\phi(x)$ with a matrix $A$ corresponds to a weighted selection of $rank(A)$-many features in parallel (e.g., projection matrices on d-dimensional subspaces correspond to the selection of $d$ many features) justifying our terminology considering a matrix $A$ as a feature selection and calling such $A$ a \defemph{feature matrix} in the following. %The same way that, for a sample input $x$, non-activated neurons $\phi_j(x)=0$ are considered as non-expressed features, we call a selection of features defined by matrix $A$ as \defemph{non-expressed} whenever $A\phi(x)=0$.


\paragraph{Distributions on feature matrices induce distributions on the feature space %via multiplication.
}\label{sct:inducingDistributions} Feature robustness is  defined in terms of feature matrices, while the interpolation approach exploiting representative data from Section~\ref{sct:representativeness} considers distributions on feature vectors, cf.~\eqref{eq:interpolating}. To connect feature robustness to the notion of $\epsilon$-interpolation, we specify for any distribution $\Acal$ on matrices $A\in \RR^{m\times m}$ an $|S|$-tuple $\Lambda_{\mathcal{A}}=(\lambda_i)$ of probability density functions $\lambda_i$ on the feature space $\RR^m$ with support containing the origin. Multiplication of a feature matrix with a feature vector $\phi(x_i)$ defines a feature direction $A\phi(x_i)$, and for each $z\in \RR^m$ there is some feature matrix $A$ with $\phi(x_i)+z=\phi(x_i)+A\phi(x_i)$ (unless $\phi(x_i)=0)$). Our choice for distributions $\lambda_i$ on $\RR^m$ are therefore distributions that are induced via multiplication of feature vectors $\phi(x_i)\in \RR^m$ with matrices $A\in \RR^{m\times m}$ sampled from a distribution on feature matrices $\Acal$ . Formally, we assume that a Borel measure $\mu_A$ is defined by a probability distribution $\mathcal{A}$ on matrices $\RR^{m\times m}$. We then define Borel measures $\mu_i$ on $\RR^m$ by $\mu_i(C)=\mu_A(\{ A\ |\ A\phi(x_i)\in C\})$ for Borel sets $C\subseteq \RR^m$. Then $\lambda_i$ is the probability distribution defined by the Borel measure $\mu_i$. As a result, we have for each $i$ that
\[ \Exp{A \sim \mathcal{A}}{\loss(\psi(\w,\phi(x_i)+  A\phi(x_i), y_i))} =  \Exp{z \sim \lambda_i}{\loss(\psi(\w,\phi(x_i)+  z, y_i))}\]


\paragraph{Example: Truncated isotropic normal distributions}\hspace{-0.2cm}are induced by a suitable distribution on feature matrices.
%The paper considers an $|S|$-tuple of densities $\Lambda_{\delta,\mathcal{A}}$ induced by  a distribution on feature matrices are truncated scaled normal distributions with support around the training samples. 
We consider probability distributions $\mathcal{K}_{\delta ||\phi(x_i)||}$
%\begin{equation}\label{eq:kernelExample}
%\lambda_i=\mathcal{K}_{\delta||\phi(x_i)||}
%\end{equation} 
on feature vectors $z\in\RR^m$ in the feature space defined by densities $k_{\delta||\phi(x_i)||}(0,z)$ with smooth rotation-invariant kernels, bounded support and bandwidth $h$:
\begin{equation}\label{eq:kernel} k_h(z_i,z)= \frac{1}{h^m}\cdot k \left (\frac{||z_i-z||}{h} \right)  \cdot \mathbbm{1}_{||z_i-z||<h}  \end{equation}
with $\mathbbm{1}_{||z_i-z||<h}=1$ when $||z-z_i||< h$ and $0$ otherwise, and such that $\int_{z\in \RR^m} k_h(z_0,z)\ dz=1\text{ for all $z_0$} .$ 
An example for such a kernel is a truncated isotropic normal distribution with variance $\delta^2 \sigma^2I$, 
$k_h(z_i,z)= \mathcal{N}(z_i, h^2\sigma^2)(z)$.
%\begin{equation}\label{eq:scaledTruncatedGaussians}
%     k_h(z_i,z)= \mathcal{N}(z_i, h^2\sigma^2)(z) =  \frac{C}{h^m} \cdot \exp\left(- \frac{||z-z_i||^2}{h^2\sigma^2}\right )  \cdot \mathbbm{1}_{||z_i-z||<h} 
% \end{equation}
%where $C$ is a normalizing constant, or the truncated multivarite Epanechnikov kernel (see e.g.~\cite{silverman1986density}). 
The following result uses that the densities in \eqref{eq:kernel} can indeed be induced by distributions on feature matrices, which enables to connect feature robustness with $\epsilon$-interpolation. 

\begin{proposition}\label{prp:lambdaA}
Let $S^\phi=\{\phi(x_i)\ |x_i\in S\}$ be a set of feature vectors in $\RR^m$. With $k_h$ defined as in \eqref{eq:kernel}, let $\lambda_i(z)=k_{\delta||\phi(x_i)||}(0,z)$ define an $|S|$-tuple $\Lambda_{\delta}$ of densities. Then there exists a distribution $\mathcal{A}_\delta$ on matrices in $\RR^{m\times m}$ of norm less than $\delta$
%that induces  each $\lambda_i$ by multiplication with $\phi(x_i)$ so that $\Lambda_{\delta,\mathcal{A}}=\Lambda$.
such that for each $i=1,\ldots,|S|$,
\[ \Exp{A\sim \mathcal{A}_\delta}{  \loss(\psi(\w,\phi(x_i)+A\phi(x_i)),y_i)}= \mathbb{E}_{\xi \sim \lambda_i}\left[\loss( \psi(\w,\phi(x_i)+ \xi),y_i)\right ] \]
\end{proposition}

The technical proof is deferred to the appendix, but we describe the distribution $\mathcal{A}$ on matrices for later use: The desired distribution is defined on the set of matrices of the form $rO$ for a real number $r$ and an orthogonal matrix $O$ (i.e. $OO^T=O^TO=I$) as a product measure combining the (unique) Haar measure on the set of orthogonal matrices $\mathcal{O}(m)$ with a suitable distribution on $\RR$. The Haar measure on $\mathcal{O}(m)$ induces the uniform measure on a sphere of radius $r$ via multiplication with a vector of radius $r$ \citep{Krantz}, and we choose a  measure on $\RR$ to match the radial change of the kernel $k_h$.



\paragraph{Feature robustness and generalization.}
With the above construction, for $\Lambda_{\mathcal{A}_\delta}$ a distribution on the feature space induced by a distribution $\mathcal{A}_\delta$ on feature matrices of norm smaller than $\delta$  (for example the distribution from Proposition~\ref{prp:lambdaA}) we have that
\begin{equation}\label{eq:splitError}
\Ecal(f) = \Ecal_{Emp}(f,S) + Int^\phi(f,S,\Lambda_{\mathcal{A}_\delta}) + \mathcal{F}(f,S, \Acal_\delta)
\end{equation}
Here, $\mathcal{A}_\delta$ can be any distribution on feature matrices and can be chosen suitably to control how well the corresponding mixture of local distributions interpolates the true distribution. The third summand is then described by how robust the model is in expectation over feature changes for $A\sim\mathcal{A}_\delta$.   In particular, if $Int^\phi(f,S,\Lambda_{\mathcal{A}_\delta})\approx 0$, then $\Ecal_{gen}(f,S)\approx \mathcal{F}(f,S, \Acal_\delta)$ and the generalization gap is determined by feature robustness.  



==> sec_oldold_representativeness.tex <==

\section{Representativeness}\label{sct:representativeness}



We begin by formalizing when a sample set $S$ is representative for a data distribution $\Dcal$.  Since neural networks are deterministic models, they can only model degenerate distributions with deterministic response variable $y$ in $\Ycal$ given $x\in \Xcal$, which entails an unavoidable error on general distributions $\Dcal$. We therefore assume the existence of an optimal label function $y(x)$. Depending on the loss function and learning task, $y(x)$ could be the conditional mean for squared loss in regression or $y(x)$ could be the Bayes classifier for the zero-one loss~\citep[cf.][]{belkinPerfectFit}. The marginal distribution $\Dcal_\Xcal$ on $\Xcal$ and the optimal label $y(x)$ define a degenerate distribution $\Dcal_{Bayes}$ on $\Xcal\times\Ycal$, which we will identify with $\Dcal$. We further assume that the marginal distribution $\Dcal_\Xcal$ is absolute continuous with respect to the Lebesgue measure on $\Xcal$ so that the distribution $\Dcal$ is described by a density function $p_{\Dcal}(x)$. 
%For technical reasons that become apparent later, we assume that $x=0$ is not in the support of $\Dcal$, which we can always achieve by extending the input by one dimension with entry $1$ corresponding to an additive bias term after multiplication with a matrix.


\paragraph{Partitioning the input space.} We choose a partition $\{V_i\ |i=1,\ldots,|S|\}$ of $\Xcal$ such that each element of this partition $V_i$ contains exactly one of the samples $x_i$ from $S$. The distribution can then be described by a set of densities $p_i(x)=\frac{1}{\alpha_i}\cdot p_\Dcal(x) \cdot \mathbf{1}_{V_i}(x)$ with support contained in $V_i$ (where $\mathbf{1}_{V_i}(x)=1$ if $x\in V_i$ and $0$ otherwise) and with normalizing factor $\alpha_i=\int_{V_i} p_\Dcal(x)  dx$. Then %we can write the risk as
%\[\Ecal(f) = \int p_\Dcal(x) \loss(f(x),y(x)) dx = \sum_{i=1}^n \alpha_i \int p_i(x) \loss(f(x),y(x)) dx=  \sum_{i=1}^n \alpha_i \mathbb{E}_{x\sim p_i}[ \loss(f(x,y(x))]. \]
the risk decomposes as $\Ecal(f) = \sum_{i=1}^n \alpha_i\cdot  \mathbb{E}_{x\sim p_i}[ \loss(f(x,y(x))]. $
Since $x_i\in V_i$ for each $i$, we can change variables and consider density functions $\lambda_i^*(\xi)=p_i(x_i+\xi)$ with support contained in a neighborhood around the origin of $\Xcal$. The risk then decomposes as
%\[\Ecal(f)= \int p_\Dcal(x) \loss(f(x),y(x)) dx =  \sum_{i=1}^n \alpha_i \mathbb{E}_{x\sim \lambda_i}[ \loss(f(x_i+x),y(x_i+x))]. \]
\[\Ecal(f)=  \sum_{i=1}^n \alpha_i \cdot \mathbb{E}_{\xi\sim \lambda_i^*}[ \loss(f(x_i+\xi),y(x_i+\xi))] %\ \text{ , where }\alpha_i^*=\int_{\Xcal} \lambda_i^*(x)  dx
.\]
Starting from this identity, we formalize an approximation to the risk. Given a sample set $S$ and an $|S|$-tuple $\Lambda = (\lambda_i)_{1\leq i\leq |S|}$ of ``local'' probability density functions on $\Xcal$ with support  ${supp}(\lambda_i)$ contained in a neighborhood around the origin, we call the pair $(S,\Lambda)$ \defemph{ $\epsilon$-representative for $\Dcal$} with respect to a model $f$ and loss $\loss$ if $|Rep^*(f,S,\Lambda) |\leq \epsilon$, where 
\begin{equation}\label{eq:representativeness}
     Rep^*(f,S,\Lambda)= \Ecal(f)   -\sum_{i=1}^n \beta_i \cdot \mathbb{E}_{\xi\sim \lambda_i}[ \loss(f(x_i+\xi),y(x_i+\xi))].
\end{equation}
and $\beta_i=\int_{\xi \in {supp}(\lambda_i)} p_\Dcal(x_i+\xi)  d\xi$. 

If the distributions $\lambda_i=\lambda_i^*$ are chosen optimal for each $i$, then $Rep^*(f,S,\Lambda)=0$. If the support of each $\lambda_i$ is decreased to the origin so that $\lambda_i=\delta_{0}$, then $Rep^*(f,S,\Lambda)=\Ecal_{gen}$ is the generalization gap. For density functions with an intermediate support, the generalization gap can be decomposed into representativeness and a term describing properties of the model around the training samples:
\[\Ecal_{gen}(f,S) = Rep^*(f,S,\Lambda)+  \sum_{i=1}^n \beta_i \cdot \Big (\mathbb{E}_{\xi\sim \lambda_i}[ \loss(f(x_i+\xi),y(x_i+\xi))-\loss(f(x_i),y(x_i))]\Big  )\]
The main idea of our approach to generalization is to take advantage of this equality and to control both representativeness and local properties of the model for a suitable $|S|$-tuple of distributions $\Lambda$
%Formally, given a family $(\lambda_i)_{1\leq i\.leq N}$ of local probability distributions (i.e., with support contained in a $\delta$-neighborhood around the origin) on $\RR^m$, the pair $(S,\Lambda_\delta)$ is called \defemph{ $\epsilon$-representative for $\Dcal$} (in feature space $\RR^m$ with respect to a model $f=(\psi\circ \phi$) and loss $\loss$) if $|Rep(f,S,\Lambda) |\leq \epsilon$, where 
%\begin{equation}\label{eq:representativeness}
%     Rep(f,S,\Lambda)= \Ecal(f)   -\sum_{(x_i,y_i)\in S} \alpha_i \cdot  \displaystyle\mathop{\mathbb{E}}_{\xi \sim \lambda_i}\left[\loss( \psi(\phi(x_i)+ \xi),y(x_i+\xi))\right]
%\end{equation}



%Formally, given a family $(\lambda_i)_{1\leq i\leq N}$ of local probability distributions (i.e., with support contained in a $\delta$-neighborhood around the origin) on $\RR^m$, the pair $(S,\Lambda_\delta)$ is called \defemph{ $\epsilon$-representative for $\Dcal$} (in feature space $\RR^m$ with respect to a model $f=(\psi\circ \phi$) and loss $\loss$) if $|Rep(f,S,\Lambda) |\leq \epsilon$, where 
%\begin{equation}\label{eq:representativeness}
%     Rep(f,S,\Lambda)= \Ecal(f)   -\sum_{(x_i,y_i)\in S} \alpha_i \cdot  \displaystyle\mathop{\mathbb{E}}_{\xi \sim \lambda_i}\left[\loss( \psi(\phi(x_i)+ \xi),y(x_i+\xi))\right]
%\end{equation}

\paragraph{A more practical version.}  We define a more practical version of the above theoretical notion of representativeness. The distribution $p_\Dcal$ is unknown and hence, in the decomposition \eqref{eq:representativeness}, we have unknown densities $\lambda_i$, unknown factors $\alpha_i$, and, in the standard setting of machine learning, we do not know how the optimal response variable $y(x_i+\xi)$ changes from $y(x_i)=y_i$. We assume that each neighborhood contributes equally to the loss, i.e., we approximate each $\alpha_i$ with $\frac 1n$. Relying on the information obtained through $S$, we could assume  that $y(x_i)\approx y_i$ int the support of the local distribution $\lambda_i$ for all training samples $(x_i,y_i)\in S$. In fact, this will allow us later to connect generalization to flatness. Alternatively, potential prior assumptions on how labels change in neighborhoods of training points could be applied. We carry on with the more general version and do not make any further restrictions for now. Our revised version of representativeness is given by
\begin{equation}\label{eq:interpolating}
     Rep(f,S,\Lambda)= \Ecal(f)   - \sum_{(x_i,y_i)\in S} \frac 1n\cdot \mathbb{E}_{\xi \sim \lambda_i}\left[\loss( f(x_i+ \xi),y_i(x_i+\xi_i)\right]
\end{equation}

\paragraph{Feature space considerations}An interesting aspect of $\epsilon$-representativeness is that it can be considered in a feature space instead of the input space. For a model $f=(\psi\circ \phi) :\Xcal\rightarrow \Ycal$, we can consider $\phi$ as a feature extractor and $\psi$ as the model, and apply our notion to the feature layer. This leads to the notion of $\epsilon$-representativeness in feature space defined for an $|S|$-tuple $\Lambda^\phi =(\lambda^\phi_i)_{1\leq i\leq N}$ of densities on $\phi(\Xcal)$ by replacing $x_i$ with $\phi(x_i)$ in \eqref{eq:interpolating}, which we denote by  $Rep^\phi(f,S,\Lambda^\phi)$.
%by  
%\begin{equation}\label{eq:representativenessFeature}
%     Int^\phi(f,S,\Lambda^\phi)= \Ecal(f)   -\frac 1n \sum_{(x_i,y_i)\in S} \mathbb{E}_{\xi \sim \lambda_i^\phi}\left[\loss( \psi(\phi(x_i)+ \xi),y_i)\right]
%\end{equation}
We can now decompose the risk  $\Ecal(f)$ of $f=(\psi\circ \phi)$ into
\[ \Ecal_{emp}(f) + Rep^\phi(f,S,\Lambda^\phi) + \left(\frac 1n \sum_{(x_i,y_i)\in S} \mathbb{E}_{\xi \sim \lambda_i^\phi}\left[\loss( \psi(\phi(x_i)+ \xi),y(x_i+\xi_i))- \loss(f(x_i),y_i) \right] \right ) \]
%\begin{wrapfigure}{h}{0.5\textwidth}
%	\centering
%	\input{images/functionIllustration}
%	\caption{Illustration of the decomposition into a feature extractor and a model, i.e., $f=\psi\circ\phi$, for neural networks.}
%	\label{fig:functionIllustration}
%\end{wrapfigure}
The term in the final bracket is determined by how the loss changes under small perturbations in the feature space for the samples in $S$.  As before,  for $\lambda_i=\delta_0$  the term in the bracket vanishes and $Rep^\phi(f,S,\Lambda)=\Ecal_{gen}$.  But the decomposition becomes more interesting for distributions with support of nonzero measure around the origin. %Having trained a neural network to a local minimizer of the empirical error, the term in the bracket is positive for neighborhoods with support of positive measure. 
 If the true distribution can be interpolated efficiently in feature space from the samples in $S$ with suitable $\lambda_i^\phi$ so that  $Rep^\phi(f,S,\lambda)\approx 0$, then the bracket approximately equals the generalization gap and the generalization gap can be estimated from local properties in feature space  around training samples. In the next section, we will define a novel notion of feature robustness of a model that is able to exploit the above connection between $\epsilon$-interpolation and the generalization gap for natural distributions $\Lambda$, 
 %. This notion of feature robustness naturally describes properties of the loss surface as a function of the weight parameters, 
%which finally allows us to connect generalization to a measure of flatness of the loss surface.


==> sec_oldoldold_representativeness.tex <==

\section{Representativeness and Interpolatingness}\label{sct:representativeness}



We begin by formalizing when a sample set $S$ is representative for a data distribution $\Dcal$.  Since neural networks are deterministic models, they can only model degenerate distributions with deterministic response variable $y$ in $\Ycal$ given $x\in \Xcal$, which entails an unavoidable error on general distributions $\Dcal$. We therefore assume the existence of an optimal label function $y(x)$. Depending on the loss function and learning task, $y(x)$ could be the conditional mean for squared loss in regression or $y(x)$ could be the Bayes classifier for the zero-one loss~\citep[cf.][]{belkinPerfectFit}. The marginal distribution $\Dcal_\Xcal$ on $\Xcal$ and the optimal label $y(x)$ define a degenerate distribution $\Dcal_{Bayes}$ on $\Xcal\times\Ycal$, which we will identify with $\Dcal$. We further assume that the marginal distribution $\Dcal_\Xcal$ is absolute continuous with respect to the Lebesgue measure on $\Xcal$ so that the distribution $\Dcal$ is described by a density function $p_{\Dcal}(x)$. 
%For technical reasons that become apparent later, we assume that $x=0$ is not in the support of $\Dcal$, which we can always achieve by extending the input by one dimension with entry $1$ corresponding to an additive bias term after multiplication with a matrix.


\paragraph{Partitioning the input space.} We choose a partition $\{V_i\ |i=1,\ldots,|S|\}$ of $\Xcal$ such that each element of this partition $V_i$ contains exactly one of the samples $x_i$ from $S$. The distribution can then be described by a set of densities $p_i(x)=\frac{1}{\alpha_i}\cdot p_\Dcal(x) \cdot \mathbf{1}_{V_i}(x)$ with support contained in $V_i$ (where $\mathbf{1}_{V_i}(x)=1$ if $x\in V_i$ and $0$ otherwise) and with normalizing factor $\alpha_i=\int_{V_i} p_\Dcal(x)  dx$. Then %we can write the risk as
%\[\Ecal(f) = \int p_\Dcal(x) \loss(f(x),y(x)) dx = \sum_{i=1}^n \alpha_i \int p_i(x) \loss(f(x),y(x)) dx=  \sum_{i=1}^n \alpha_i \mathbb{E}_{x\sim p_i}[ \loss(f(x,y(x))]. \]
the risk decomposes as $\Ecal(f) = \sum_{i=1}^n \alpha_i\cdot  \mathbb{E}_{x\sim p_i}[ \loss(f(x,y(x))]. $
Since $x_i\in V_i$ for each $i$, we can change variables and consider density functions $\lambda_i^*(\xi)=p_i(x_i+\xi)$ with support contained in a neighborhood around the origin of $\Xcal$. The risk then decomposes as
%\[\Ecal(f)= \int p_\Dcal(x) \loss(f(x),y(x)) dx =  \sum_{i=1}^n \alpha_i \mathbb{E}_{x\sim \lambda_i}[ \loss(f(x_i+x),y(x_i+x))]. \]
\[\Ecal(f)=  \sum_{i=1}^n \alpha_i \cdot \mathbb{E}_{\xi\sim \lambda_i^*}[ \loss(f(x_i+\xi),y(x_i+\xi))] %\ \text{ , where }\alpha_i^*=\int_{\Xcal} \lambda_i^*(x)  dx
.\]
Starting from this identity, we formalize an approximation to the risk. Given a sample set $S$ and an $|S|$-tuple $\Lambda = (\lambda_i)_{1\leq i\leq |S|}$ of ``local'' probability density functions on $\Xcal$ with support  ${supp}(\lambda_i)$ contained in a neighborhood around the origin, we call the pair $(S,\Lambda)$ \defemph{ $\epsilon$-representative for $\Dcal$} with respect to a model $f$ and loss $\loss$ if $|Rep(f,S,\Lambda) |\leq \epsilon$, where 
\begin{equation}\label{eq:representativeness}
     Rep(f,S,\Lambda)= \Ecal(f)   -\sum_{i=1}^n \beta_i \cdot \mathbb{E}_{\xi\sim \lambda_i}[ \loss(f(x_i+\xi),y(x_i+\xi))].
\end{equation}
and $\beta_i=\int_{\xi \in {supp}(\lambda_i)} p_\Dcal(x_i+\xi)  dx$. 

If the distributions $\lambda_i=\lambda_i^*$ are chosen optimal for each $i$, then $Rep(f,S,\Lambda)=0$. If the support of all distributions is decreased to the origin so that $\lambda_i=\delta_{0}$, then $Rep(f,S,\Lambda)=\Ecal_{gen}$ is the generalization gap. For density functions with an intermediate support, the generalization gap can be decomposed into representativeness and a term describing properties of the model around the training samples:
\[\Ecal_{gen}(f,S) = Rep(f,S,\Lambda)+  \sum_{i=1}^n \beta_i \cdot \Big (\mathbb{E}_{\xi\sim \lambda_i}[ \loss(f(x_i+\xi),y(x_i+\xi))-\loss(f(x_i),y(x_i))]\Big  )\]
The main idea of our approach to generalization is to take advantage of this equality and to control both representativeness and local properties of the model for a suitable $|S|$-tuple of distributions $\Lambda$
%Formally, given a family $(\lambda_i)_{1\leq i\leq N}$ of local probability distributions (i.e., with support contained in a $\delta$-neighborhood around the origin) on $\RR^m$, the pair $(S,\Lambda_\delta)$ is called \defemph{ $\epsilon$-representative for $\Dcal$} (in feature space $\RR^m$ with respect to a model $f=(\psi\circ \phi$) and loss $\loss$) if $|Rep(f,S,\Lambda) |\leq \epsilon$, where 
%\begin{equation}\label{eq:representativeness}
%     Rep(f,S,\Lambda)= \Ecal(f)   -\sum_{(x_i,y_i)\in S} \alpha_i \cdot  \displaystyle\mathop{\mathbb{E}}_{\xi \sim \lambda_i}\left[\loss( \psi(\phi(x_i)+ \xi),y(x_i+\xi))\right]
%\end{equation}



%Formally, given a family $(\lambda_i)_{1\leq i\leq N}$ of local probability distributions (i.e., with support contained in a $\delta$-neighborhood around the origin) on $\RR^m$, the pair $(S,\Lambda_\delta)$ is called \defemph{ $\epsilon$-representative for $\Dcal$} (in feature space $\RR^m$ with respect to a model $f=(\psi\circ \phi$) and loss $\loss$) if $|Rep(f,S,\Lambda) |\leq \epsilon$, where 
%\begin{equation}\label{eq:representativeness}
%     Rep(f,S,\Lambda)= \Ecal(f)   -\sum_{(x_i,y_i)\in S} \alpha_i \cdot  \displaystyle\mathop{\mathbb{E}}_{\xi \sim \lambda_i}\left[\loss( \psi(\phi(x_i)+ \xi),y(x_i+\xi))\right]
%\end{equation}

\paragraph{A more practical version.} For applicability to the standard setting of machine learning, we define a more practical version of the above theoretical notion of representativeness that is based only on the information obtained from the sample set $S$. The distribution $p_\Dcal$ is unknown and hence, in the decomposition \eqref{eq:representativeness}, we have unknown densities $\lambda_i$, unknown factors $\alpha_i$, and we do not know how the optimal response variable $y(x_i+\xi)$ changes from $y(x_i)$.  Having to rely on interpolation from local information, we suppose that  \textcolor{blue}{$y(x_i)\approx y_i$} for all training samples $(x_i,y_i)\in S$ and we assume that each neighborhood contributes equally to the loss, i.e., we approximate each $\alpha_i$ with $\frac 1n$, and we assume the support of the local distribution to be sufficiently small to justify \textcolor{blue}{approximately} locally constant label $y(x_i+\xi)=y_i$. 
%:
%\[  \sum_{i=1}^n \alpha_i\cdot \mathbb{E}_{\xi\sim \lambda_i}[ \loss(f(x_i+\xi),y(x_i+\xi))] \approx  \sum_{i=1}^n  \frac 1n\cdot  \mathbb{E}_{\xi\sim \lambda_i}[ \loss(f(x_i+\xi),y_i)] \] 
Given an $|S|$-tuple $\Lambda =(\lambda_i)_{1\leq i\leq N}$ of densities on $\Xcal$ with support contained in a neighborhood around the origin, the pair $(S,\Lambda)$ is called \defemph{ $\epsilon$-interpolating for $\Dcal$} with respect to a model $f$ and loss $\loss$, if $|Int(f,S,\Lambda) |\leq \epsilon$, where 
\begin{equation}\label{eq:interpolating}
     Int(f,S,\Lambda)= \Ecal(f)   - \sum_{(x_i,y_i)\in S} \frac 1n\cdot \mathbb{E}_{\xi \sim \lambda_i}\left[\loss( f(x_i+ \xi),y_i)\right]
\end{equation}
Although the label $y(x_i+\xi)$ is not known in practical settings, we will investigate in \textcolor{red}{Appendix}~\ref{sct:labelChanges} the consequences from dropping the assumption of \textcolor{blue}{approximately} locally constant labels.


\paragraph{Feature space considerations}An interesting aspect of the notions $\epsilon$-representativeness and $\epsilon$-interpolation is that both can be considered in a feature space instead of the input space. For a model $f=(\psi\circ \phi) :\Xcal\rightarrow \Ycal$, we can consider $\phi$ as a feature extractor and $\psi$ as the model, and apply our notions to the feature layer. This leads to the notion of $\epsilon$-interpolation in feature space defined for an $|S|$-tuple $\Lambda^\phi =(\lambda^\phi_i)_{1\leq i\leq N}$ of densities on $\phi(\Xcal)$ by replacing $x_i$ with $\phi(x_i)$ in \eqref{eq:interpolating}, which we denote by  $Int^\phi(f,S,\Lambda^\phi)$.
%by  
%\begin{equation}\label{eq:representativenessFeature}
%     Int^\phi(f,S,\Lambda^\phi)= \Ecal(f)   -\frac 1n \sum_{(x_i,y_i)\in S} \mathbb{E}_{\xi \sim \lambda_i^\phi}\left[\loss( \psi(\phi(x_i)+ \xi),y_i)\right]
%\end{equation}
We can now decompose the risk of $f=(\psi\circ \phi)$ into
\[  \Ecal(f) = \Ecal_{emp}(f) + Int^\phi(f,S,\Lambda^\phi) + \left(\frac 1n \sum_{(x_i,y_i)\in S} \mathbb{E}_{\xi \sim \lambda_i^\phi}\left[\loss( \psi(\phi(x_i)+ \xi),y_i)- \loss(f(x_i),y_i) \right] \right ) \]
%\begin{wrapfigure}{h}{0.5\textwidth}
%	\centering
%	\input{images/functionIllustration}
%	\caption{Illustration of the decomposition into a feature extractor and a model, i.e., $f=\psi\circ\phi$, for neural networks.}
%	\label{fig:functionIllustration}
%\end{wrapfigure}
The term in the final bracket is determined by how the loss changes under small perturbations in the feature space for the samples in $S$.  As before,  for $\lambda_i=\delta_0$  the term in the bracket vanishes and $Int^\phi(f,S,\Lambda)=\Ecal_{gen}$.  But the decomposition becomes more interesting for distributions with support of nonzero measure around the origin. %Having trained a neural network to a local minimizer of the empirical error, the term in the bracket is positive for neighborhoods with support of positive measure. 
 If the true distribution can be interpolated efficiently in feature space from the samples in $S$ with suitable $\lambda_i^\phi$ so that  $Int^\phi(f,S,\lambda)\approx 0$, then the bracket approximately equals the generalization gap and the generalization gap can be estimated from local properties in feature space  around training samples. In the next section, we will define a novel notion of feature robustness of a model that is able to exploit the above connection between $\epsilon$-interpolation and the generalization gap for natural distributions $\Lambda$, 
 %. This notion of feature robustness naturally describes properties of the loss surface as a function of the weight parameters, 
%which finally allows us to connect generalization to a measure of flatness of the loss surface.


==> sec_relatedWork.tex <==
\section{Related Work}\label{sec:relatedWork}
